Double Beta Decay APPEC Committee Report

This report constitutes the roadmap document prepared by the Double Beta Decay APPEC Committee for the APPEC SAC on the future neutrinoless double beta decay experimental programme in Europe. It reviews the existing, planned and proposed technologies for neutrinoless double beta decay, their discovery potential and technical challenges, making a critical examination of resources and schedules. It also provides a concise discussion of the theoretical issues and of the status and uncertainties on the nuclear matrix element evaluation.

==> NextLatexPackagesBase.tex <==
\usepackage{babel}
\usepackage[document]{ragged2e}

\usepackage{amsfonts}
\usepackage{wrapfig}
\usepackage{hyperref}

\usepackage{graphbox}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{amsmath,amssymb, gensymb}
\usepackage{natbib,hyperref}
\usepackage{url}
\usepackage{siunitx}
\sisetup{separate-uncertainty=true}
\usepackage{xspace}
\usepackage{microtype}
\usepackage{subfig}
\usepackage[useregional]{datetime2}
\usepackage{graphicx}
%\usepackage{subcaption}


==> tcbraster.code.tex <==
%% The LaTeX package tcolorbox - version 4.21 (2019/09/19)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2019 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{4.21}

\newcounter{tcbrastercolumn}
\newcounter{tcbrasterrow}
\newcounter{tcbraster}

\newrobustcmd{\thetcbrasternum}{\the\numexpr(\c@tcbrasterrow-1)*\kvtcb@raster@columns+\c@tcbrastercolumn\relax}

\def\tcb@raster@ehg@all{%
  \tcbset{equal height group={\kvtcb@raster@ehgid}}%
}

\def\tcb@raster@ehg@row{%
  \tcbset{equal height group={\kvtcb@raster@ehgid @\number\c@tcbrasterrow}}%
}


\tcbset{%
  raster columns/.store in=\kvtcb@raster@columns,
  raster rows/.store in=\kvtcb@raster@rows,
  raster width/.store in=\kvtcb@raster@width,
  raster height/.store in=\kvtcb@raster@height,
  %
  raster before skip/.store in=\kvtcb@raster@skip@before,
  raster after skip/.store in=\kvtcb@raster@skip@after,
  raster left skip/.store in=\kvtcb@raster@skip@left,
  raster right skip/.store in=\kvtcb@raster@skip@right,
  %
  raster column skip/.store in=\kvtcb@raster@xskip,
  raster row skip/.store in=\kvtcb@raster@yskip,
  %
  raster equal skip/.style={raster before skip=#1,raster after skip=#1,
    raster column skip=#1,raster row skip=#1},
  %
  raster@halign/.store in=\kvtcb@raster@halign,
  raster halign/.is choice,
  raster halign/center/.style={raster@halign=\centering},
  raster halign/left/.style={raster@halign=\raggedright},
  raster halign/right/.style={raster@halign=\raggedleft},
  %
  raster valign/.store in=\kvtcb@raster@valign,
  %
  raster equal height group/.store in=\kvtcb@raster@ehgid,%
  raster equal height/.is choice,
  raster equal height/.default=all,
  raster equal height/none/.code={\let\tcb@raster@ehg@set\@empty},%
  raster equal height/rows/.code={\let\tcb@raster@ehg@set\tcb@raster@ehg@row},%
  raster equal height/all/.code={\let\tcb@raster@ehg@set\tcb@raster@ehg@all},%
  %
  raster force size/.is choice,%
  raster force size/.default=true,%
  raster force size/true/.code={\let\tcb@raster@set@size\tcbset@late@options},%
  raster force size/false/.code={\let\tcb@raster@set@size\tcbset},%
  raster multicolumn/.code={%
    \ifnum\numexpr\c@tcbrastercolumn+#1>\numexpr\kvtcb@raster@columns+1\relax
      \tcb@warning{'raster multicolumn' combined too much columns}%
    \else%
      \tcbset@late@options{%
        code={\preto\kvtcb@afterbox{\addtocounter{tcbrastercolumn}{\numexpr#1-1}}},
        width=(\tcb@raster@box@width+\tcb@raster@xskip)*#1-\tcb@raster@xskip}%
    \fi%
  },
  raster multirow/.code={%
    \ifdefined\tcb@raster@box@height%
      \tcbset@late@options{%
        height=(\tcb@raster@box@height+\tcb@raster@yskip)*#1-\tcb@raster@yskip}%
    \else%
      \tcb@warning{'raster multirow' needs a fixed 'raster height'}%
    \fi%
  },
  raster width center/.style={raster width=\linewidth,raster left skip=(\linewidth-(#1))/2,raster right skip=(\linewidth-(#1))/2},
  raster width flush left/.style={raster width=\linewidth,raster left skip=0pt,raster right skip=\linewidth-(#1)},
  raster width flush right/.style={raster width=\linewidth,raster left skip=\linewidth-(#1),raster right skip=0pt},
}

\tcbset{
  raster reset/.style={
    raster width=\linewidth,raster height=0pt,
    raster equal skip=2mm,
    raster columns=2,raster rows=2,
    raster left skip=0pt,raster right skip=0pt,
    raster halign=left,raster valign=center,
    raster equal height=none,
    raster equal height group={REG@\tcb@raster@number},
    raster force size,},
  raster reset
}

\setcounter{tcbraster}{0}

\let\tcb@raster@change@minipage\@empty
\let\tcb@raster@change@fitbox\@empty
\def\tcb@raster@change@hbox{\tcbset{capture=minipage}}

\def\tcb@height@fill@unbroken@raster#1{%
  \ifnum\c@tcblayer<2\relax%
    \kvtcb@beforebox%
    \def\kvtcb@beforebox{}%
    \tcb@breakat@init%
    \tcbset{compress page=#1}%
    \tcb@comp@h@page%
    \ifdim\tcb@h@page<0pt\relax\unkern\pagebreak\tcb@comp@h@page\kern\tcb@raster@skip@left\fi%
    \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand}%
  \fi%
}

\newenvironment{tcbraster}[1][]{%
  \tcb@layer@pushup%
  \stepcounter{tcbraster}%
  \edef\tcb@raster@number{\number\c@tcbraster}%
  \edef\tcb@raster@save@column{\number\c@tcbrastercolumn}%
  \edef\tcb@raster@save@row{\number\c@tcbrasterrow}%
  \let\tcb@raster@change@fitbox\@empty%
  \setcounter{tcbrastercolumn}{1}%
  \setcounter{tcbrasterrow}{1}%
  \let\tcb@height@fill@unbroken\tcb@height@fill@unbroken@raster%
  \tcbset{every box on layer \the\numexpr\number\c@tcblayer+1\relax/.code={%
    \tcb@raster@ehg@set%
    \tcbset{raster every box/.try}%
    \ifodd\c@tcbrastercolumn\relax%
      \tcbset{raster odd column/.try}%
    \else%
      \tcbset{raster even column/.try}%
    \fi%
    \tcbset{raster column \number\c@tcbrastercolumn/.try}%
    \ifodd\c@tcbrasterrow\relax%
      \tcbset{raster odd row/.try}%
    \else%
      \tcbset{raster even row/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow/.try}%
    \ifodd\thetcbrasternum\relax%
      \tcbset{raster odd number/.try}%
    \else%
      \tcbset{raster even number/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow\space column \number\c@tcbrastercolumn/.try}%
    \tcbset{raster number \thetcbrasternum/.try}%
  }}%
  \tcbset{#1}%
  % sanitize
  \tcbdimto\tcb@raster@width{\kvtcb@raster@width}%
  \tcbdimto\tcb@raster@height{\kvtcb@raster@height}%
  \tcbdimto\tcb@raster@skip@before{\kvtcb@raster@skip@before}%
  \tcbdimto\tcb@raster@skip@after{\kvtcb@raster@skip@after}%
  \tcbdimto\tcb@raster@skip@left{\kvtcb@raster@skip@left}%
  \tcbdimto\tcb@raster@skip@right{\kvtcb@raster@skip@right}%
  \tcbdimto\tcb@raster@xskip{\kvtcb@raster@xskip}%
  \tcbdimto\tcb@raster@yskip{\kvtcb@raster@yskip}%
  \tcbset@late@options{%
    before={\ifhmode\unskip\fi\ifnum\c@tcbrastercolumn>1 \kern\tcb@raster@xskip\else%
      \ifnum\c@tcbrasterrow>1 \parindent\z@\parskip\z@\par\nointerlineskip\addvspace{\the\dimexpr\tcb@raster@yskip\relax}\noindent\fi%
      \kern\tcb@raster@skip@left\fi},
    after={%
      \ifnum\c@tcbrastercolumn=\kvtcb@raster@columns\relax%
        \kern\tcb@raster@skip@right%
        \setcounter{tcbrastercolumn}{1}\addtocounter{tcbrasterrow}{1}%
      \else%
        \stepcounter{tcbrastercolumn}%
      \fi},%
    box align=\kvtcb@raster@valign,%
  }%
  \tcbdimto\tcb@raster@box@width{(\tcb@raster@width+\tcb@raster@xskip-\tcb@raster@skip@left-\tcb@raster@skip@right)/\kvtcb@raster@columns-\tcb@raster@xskip}%
  \tcb@raster@set@size{%
    code={\csuse{tcb@raster@change@\kvtcb@capture}},
    width=\tcb@raster@box@width,
  }%
  \ifdim\dimexpr\tcb@raster@height>0pt\relax%
    \tcbdimto\tcb@raster@box@height{(\tcb@raster@height+\tcb@raster@yskip-0.001pt)/\kvtcb@raster@rows-\tcb@raster@yskip}%
    \tcb@raster@set@size{height=\tcb@raster@box@height}%
  \fi%
  \let\tcb@end@raster\@empty%
  \ifinner\ifhmode%
    \color@vbox%
    \hsize=\tcb@raster@width%
    \let\tcb@end@raster\color@endbox%
  \fi\fi%&
  \if@nobreak%
    \iftcb@ignorenobreak%
      {\par\nointerlineskip%
      \addvspace{\glueexpr\tcb@raster@skip@before-\parskip}}%
    \fi%
  \else%
    {\par\nointerlineskip%
    \addvspace{\glueexpr\tcb@raster@skip@before-\parskip}}%
  \fi%
  \tcb@parfillskip@check\kvtcb@raster@halign\noindent%
}{%
  \ifhmode\unskip\fi%
  \ifnum\c@tcbrastercolumn>1 %
    \kern\tcb@raster@skip@right%
  \fi%
  \begingroup%
  \par\nointerlineskip%
  \addvspace{\glueexpr\tcb@raster@skip@after-\parskip}%
  \endgroup%
  \tcb@end@raster%
  \setcounter{tcbrastercolumn}{\tcb@raster@save@column}%
  \setcounter{tcbrasterrow}{\tcb@raster@save@row}%
}

\newcommand{\tcbitem@following}[1][]{%
  \end{tcolorbox}\begin{tcolorbox}[#1]%
}

\newcommand{\tcbitem@first}[1][]{%
  \let\tcbitem=\tcbitem@following%
  \begin{tcolorbox}[#1]%
}

\newenvironment{tcbitemize}[1][]{%
  \begin{tcbraster}[#1]%
  \let\tcb@raster@change@fitbox=\tcb@raster@change@hbox%
  \let\tcbitem=\tcbitem@first%
}{\end{tcolorbox}\end{tcbraster}}

\newenvironment{tcboxedraster}[2][]{%
  \tcolorbox[#2]\begin{tcbraster}[#1]}%
  {\end{tcbraster}\endtcolorbox}

\newenvironment{tcboxeditemize}[2][]{%
  \tcolorbox[#2]\tcbitemize[#1]}%
  {\endtcbitemize\endtcolorbox}

